Automatic Detection of Entity-Manipulated Text using Factual Knowledge

In this work, we focus on the problem of distinguishing a human written news article from a news article that is created by manipulating entities in a human written news article (e.g., replacing entities with factually incorrect entities). Such manipulated articles can mislead the reader by posing as a human written news article. We propose a neural network based detector that detects manipulated news articles by reasoning about the facts mentioned in the article. Our proposed detector exploits factual knowledge via graph convolutional neural network along with the textual information in the news article. We also create challenging datasets for this task by considering various strategies to generate the new replacement entity (e.g., entity generation from GPT-2). In all the settings, our proposed model either matches or outperforms the state-of-the-art detector in terms of accuracy. Our code and data are available at https://github.com/UBC-NLP/manipulated_entity_detection.

==> discussion.tex <==
\subsection{Discussion}
\label{sec:discssion}

We summarize our findings from this project and present our thoughts for further research on this problem.

\begin{itemize}
  \item The current state-of-the-art detector that rely mostly on textual knowledge can benefit from explicitly modeling the factual knowledge. Our project scratch the surface of principled approaches to construct the factual knowledge underlying the document with two approaches: triplets from knowledge base and entity co-occurrence graph.
  \item Our proposed algorithm to utilize the state-of-the-art text generative model, GPT-2 seems to utilize the context of the news article to generate replacement entity. However, the GPT-2 based replacement strategy did not make the detection task harder. We conjecture that our proposed algorithm might introduce distributional artifacts in the manipulated text, which is easier for the detectors to pick up on. We expect advances in text generative models can mitigate this artifact issue. Towards this goal, we posit a  promising direction to improve our proposed algorithm can be to consider bidirectional context (context to the left and to the right of the token to be perturbed) while generating the replacement entity.
  \item Factual knowledge constructed using triplets from knowledge bases can suffer from knowledge noise issues, which can negatively affect the detection performance of our proposed detector. Our experimentation with randomly sampling a subset of triplets for each entity to minimize the noise introduced by popular entities which might have more KB triplets did not provide improved results. We suspect a principled way to select the triplets relevant to a given entity in a document is needed to resolve the knowledge noise issue. Towards this goal, one promising step in this direction can be to automatically identify the important triplets from candidate triplets based on the context of the news article using techniques such as cross-attention~\cite{vaswani_neurips17}.
  \item There might be alternative methods to construct factual knowledge which do not suffer from knowledge noise issue. Instead of considering only the one hop neighbors for each document entity, we can query the knowledge base for paths connecting different document entities and integrate these paths into the textual detector. We can also extract the facts from the news article using information extraction systems like OpenIE~\cite{angeli-etal-2015-leveraging} and integrate these facts into the textual detector. Note that the facts generated by OpenIE system are not grounded to a fixed schema and entities or relations can be erroneous.
  \item Our proposed detector relies on a simple compositionality technique of averaging to combine information from different nodes in the factual graph followed by the concatenation operation to merge the averaged node representation with RoBERTa's textual representation. We expect a principled compositionality technique such as cross-attention over node representation w.r.t. textual representation can preserve the factual information well. We also expect a tighter coupling of factual information and textual information by fusing them during intermediate layers of the graph convolutional networks and RoBERTa model can provide improved detection performance.
  \item Building fake news detector that can explain its decision is a non-trivial task. Such explainable detector can interface with humans in solving the detection task for real world applications, especially in social media platforms. Our proposed detectors achieve poor classification performance (entity classification accuracy and manipulated entity recall) in general on different manipulated text detection settings. We suspect that the loss function used for entity classification is not sensitive to the imbalanced nature of the problem. We believe penalizing the error in misclassifying samples corresponding to minority class (manipulated entity) more can improve the overall entity classification performance.
  \item This project focuses on only one type of article manipulation --- entity perturbation. It is unclear if the proposed detector can provide reasonable detection performance for other types of manipulations studied in the literature such as negation, subject-object exchange, and cause confounding. For subject-object exchange, the detector can be supervised to detect manipulated subjects and objects. It might be challenging to detect articles that undergo negation manipulation, as the manipulations are subtle and requires fine-grained linguistic knowledge (e.g., identifying strange expressions) to perform well in the detection task. Nevertheless, it's an important endeavor to build a detector that can detect a wide variety of manipulations.
  \item Our proposed entity replacement strategies focus only on three types of named entities: persons, organizations and locations. It might be interesting to consider all the types of named entities including product, date, time and so on. Building detectors to cover a wide range of types is very challenging, as some types such as numbers are harder to reason as the textual knowledge corresponding to those named entities are not accurately captured by the state-of-the-art language representation models. 
\end{itemize}

==> problem.tex <==
\section{Problem Statement}
\label{sec:ps}
Manipulated text detection can be formalized as follows. Let $\mathcal{X}$ denote the input space defined over the set of all human written news articles and the set of all news articles manipulated according to a particular manipulation technique (e.g., entity replacement with a maximum number of replacements to be 3 and the replacements are suggested by GPT-2 (see Section~\ref{sec:gpt2er})). Let $\mathcal{Y} = \{0,1\}$ denote the set of possible labels, where the label $0$ and label $1$ correspond to manipulated news article and human written news article respectively. Let $\mathcal{D}$ denote the data distribution defined over $\mathcal{X}\times\mathcal{Y}$. Let $\mathcal{L}$ denote the labeled data set, where $\mathcal{L} = \{(\mathbf{x}_i, y_i)\}_{i=1}^{n} \sim (\mathcal{D})^n$ containing samples $(\mathbf{x}_i, y_i)$ drawn i.i.d from $\mathcal{D}$. The problem of manipulated text detection is to build a classifier $f: \mathcal{X} \to \mathcal{Y}$ that achieves high accuracy on unseen examples, $ Pr_{(\mathbf{x},y)\sim\mathcal{D}} (f(\mathbf{x}) = y)$).
